Modeling lens potentials with continuous neural fields in galaxy-scale strong lenses

Strong gravitational lensing is a unique observational tool for studying the dark and luminous mass distribution both within and between galaxies. Given the presence of substructures, current strong lensing observations demand more complex mass models than smooth analytical profiles, such as power-law ellipsoids. In this work, we introduce a continuous neural field to predict the lensing potential at any position throughout the image plane, allowing for a nearly model-independent description of the lensing mass. We apply our method on simulated Hubble Space Telescope imaging data containing different types of perturbations to a smooth mass distribution: a localized dark subhalo, a population of subhalos, and an external shear perturbation. Assuming knowledge of the source surface brightness, we use the continuous neural field to model either the perturbations alone or the full lensing potential. In both cases, the resulting model is able to fit the imaging data, and we are able to accurately recover the properties of both the smooth potential and of the perturbations. Unlike many other deep learning methods, ours explicitly retains lensing physics (i.e., the lens equation) and introduces high flexibility in the model only where required, namely, in the lens potential. Moreover, the neural network does not require pre-training on large sets of labelled data and predicts the potential from the single observed lensing image. Our model is implemented in the fully differentiable lens modeling code Herculens.

==> table_notation.tex <==
\begin{table}[!h]
\caption{List of the main notations used in the paper.} \label{tab:notations}
\renewcommand{\arraystretch}{1.4}
\centering
{\small
\begin{tabular}{ll}

\hline
Notation & Definition \\
\hline\hline

\multicolumn{2}{l}{\textsl{Observation}} \\
\hline

\data & Imaging data \\
\datacovmatrix & Data covariance matrix \\
$\mathbf{n}$ & Additive noise (instrumental + read-out)\\
%$\sigma_\data$ & Data noise map $\equiv$ $\sqrt{ | {\rm diag} \left[ \datacovmatrix \right] | }$ \\

\hline
\multicolumn{2}{l}{\textsl{Model components}} \\
\hline

\model & Image model \\
\convop & Blurring operator \\
\lensingop\!(\lenspot) & Lensing operator \\
\lenspot, \source, \lenslight & Lens potential, source light, lens light \\
%\lenspotmacro & Macro lensing potential \\
%\lenspotpert & Perturbations to the lensing potential \\

\hline
\multicolumn{2}{l}{\textsl{Neural network}} \\
\hline

$\Phi$ &Neural network function \\
$\mathbf{W_n}$ &Neural network n-th weight matrix\\
$\mathbf{b_n}$ &Neural network n-th bias vector\\
$\phi$ &Neural network activation function\\
$\gamma_{\sigma}$ &Random input embedding with variance $\sigma$ \\


\hline
\multicolumn{2}{l}{\textsl{Model parametrization}} \\
\hline

\modelparam & Vector containing all parameters \\
$\boldsymbol{\eta}_{\Phi}$ &Network parameters (weights and biases)\\
$\boldsymbol{\eta}_{s}$ &Parameters for analytical source profile\\


\hline
\multicolumn{2}{l}{\textsl{Optimization \& Inference}} \\
\hline

%\likelihoodsimple & Log-likelihood \\
%$\priorsimple_\lenspotscalar$, $\priorsimple_\sourcescalar$, $\priorsimple_\lenslightscalar$ & Log-priors (regularization terms) \\
$\mathcal{L}$, $\nabla\mathcal{L}$ & Loss function and its gradient \\
$\boldsymbol{\eta}^*$ & Optimal solution  \\
$\lambda$ & Learning rate \\
\hline
\end{tabular}
}
\end{table}


==> table_sim_input.tex <==
\begin{table}[h!]
\caption{} \label{app:tab:sim_params}
\renewcommand{\arraystretch}{1.2}
\centering
{\small
\begin{tabular}{lc}
\hline
\textbf{Deflector} & \\
\hline
\ \ \ \textbf{Smooth component} (SIE) & \\
\ \ \ \ \ \ Einstein radius $\theta_{\rm E}$ [arcsec] & 1.8 \\
\ \ \ \ \ \ Ellipticity $(e_1, e_2)$ & $(0.15, -0.04)$ \\
\ \ \ \ \ \ Position (RA, Dec) [arcsec] & $(0.0, 0.0)$ \\
\hline\hline
\textbf{Perturbations to the lensing potential} & \\
\hline
\ \ \ \textbf{Dark halo} (SIE) & \\
\ \ \ \ \ \ Einstein radius $\theta_{\rm E}$ [arcsec] & 0.07 \\
\ \ \ \ \ \ Ellipticity $(e_1, e_2)$ & $(0.0, 0.0)$ \\
\ \ \ \ \ \ Position (RA, Dec) [arcsec] & $(1.9, -0.4)$ \\
\hline
\ \ \ \textbf{Gaussian random field} (GRF) & \\
\ \ \ \ \ \ Amplitude $A$ & $10^{-4}$ \\
\ \ \ \ \ \ Slope $\beta$ & $5.5$ \\
\hline
\ \ \ \textbf{External shear} & \\
\ \ \ \ \ \ First Shear component, $\gamma_{1}$ & 0.01 \\
\ \ \ \ \ \ Second Shear component, $\gamma_{2}$ & -0.03 \\
\ \ \ \ \ \ Position, (RA, Dec) [arcsec] where \\
\ \ \ \ \ \ shear deflection is 0, & $(0.0, 0.0)$ \\
\hline\hline
\textbf{Source} (S{\'e}rsic) & \\
\hline
\ \ \ \ \ \ Ellipticity $(e_1, e_2)$ & $(-0.09, 0.03)$ \\
\ \ \ \ \ \ Half-light radius $R_{\rm S}$ [arcsec] & 0.8 \\
\ \ \ \ \ \ S{\'e}rsic index $n_{\rm s}$ & 2.0 \\
\ \ \ \ \ \ Position, (RA, Dec) [arcsec] & $(0.4, 0.15)$ \\
\ \ \ \ \ \ \textcolor{red}{Surface brightness (?)} & 90.0 \\
\hline
\end{tabular}
}
\end{table}


==> table_sim_instru.tex <==
\begin{table}[h!]
\caption{} \label{app:tab:sim_settings}
\renewcommand{\arraystretch}{1.2}
\centering
{\small
\begin{tabular}{lc}
\hline
Instrument/filter & \textcolor{red}{Gaussian} \\
%\hline
Pixel size [arcsec] & 0.08 \\ 
%\hline
Exposure time [s] & 2000 \\ 
%\hline
Zero-point [mag] & 30 \\ 
%\hline
Sky brightness & 22 mag\,arcsec$^{-2}$ \\ 
%\hline
Readout noise & 4 e$^-$ \\ 
%\hline
PSF kernel & simulated with \textsc{TinyTim} \\
%\hline
Noise & readout + sky + target \\
\hline
\end{tabular}
}
\end{table}

